In Search of Metrics to Guide Developer-Based Refactoring Recommendations

Context. Source code refactoring is a well-established approach to improving source code quality without compromising its external behavior. Motivation. The literature described the benefits of refactoring, yet its application in practice is threatened by the high cost of time, resource allocation, and effort required to perform it continuously. Providing refactoring recommendations closer to what developers perceive as relevant may support the broader application of refactoring in practice and drive prioritization efforts. Aim. In this paper, we aim to foster the design of a developer-based refactoring recommender, proposing an empirical study into the metrics that study the developer's willingness to apply refactoring operations. We build upon previous work describing the developer's motivations for refactoring and investigate how product and process metrics may grasp those motivations. Expected Results. We will quantify the value of product and process metrics in grasping developers' motivations to perform refactoring, thus providing a catalog of metrics for developer-based refactoring recommenders to use.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> Section/Background.tex <==
\section{Background}
\label{sec:Background}




==> Section/Discussion.tex <==
\section{Discussion}
\label{sec:Discussion}



==> Section/Results.tex <==
\section{Results}
\label{sec:Results}


==> Tables/metrics.old.tex <==
\begin{table*}[h]
\centering
\small
% \resizebox{\textwidth}{!}{
\begin{tabular}{l|l|p{15cm}}
\hline
& \textbf{Metric} & \textbf{Description} \\ \hline 
\multirow{15}{*}{\rotatebox[origin=c]{90}{Rahman~\cite{rahm2013}}} & COMM     & The cumulative number of changes in a given file up to the considered commit.                                                  \\
                                                                              &  ADEV     &  The cumulative number of active developers who modified a given file up to the considered commit.                              \\
                                                                              & DDEV     & The cumulative number of distinct developers contributed to a given file up to the considered commit.                          \\
                                                                              &  ADD      &  The normalized number of lines added to a given file in the considered commit.                                                 \\
                                                                              & DEL      & The normalized number of lines removed from a given file in the considered commit.                                             \\
                                                                              &  OWN      &  The value indicates whether the file owner does the commit.                                                            \\
                                                                              & MINOR    & The number of contributors who contributed less than 5\% of a given file up to the considered commit.                          \\
                                                                              &  SCTR     &  The number of packages modified by the committer in the considered commit.                                                     \\
                                                                              & NADEV    & The number of active developers who changed any of the files involved in the commits where the given file has been modified.   \\
                                                                              &  NDDEV    &  The number of distinct developers who changed any of the files involved in the commits where the given file has been modified. \\
                                                                              & NCOMM    & The number of commits where the given has been involved.                                                                       \\
                                                                              &  NSCTR    &  The number of different packages touched by the developer in commits where the file has been modified.                         \\
                                                                              & OEXP     & The percentage of code lines authored by a given developer in the project.                                               \\
                                                                              &  EXP      &  The mean of the experience of all developers across the whole project.                                                         \\
\hline 
\multirow{10}{*}{\rotatebox[origin=c]{90}{Kamei~\cite{kamei2012large}}} & ND       & The number of directories involved in a commit.                                                                                \\                                       &   NS     & Number of modified subsystems.                      \\
  & NF & Number of modified files. \\

                                                                              &  ENTROPY  &  The distribution of the modified code across each given file in the considered commit.                                         \\
                                                                              & LA       & Ten number of lines added to the given file in the considered commit (absolute number of the ADD metric).                      \\
                                                                              &  LD       &  The number of lines removed from the given file in the considered commit (absolute number of the DEL metric).                  \\
                                                                              & LT       & The number of lines of code in the given file in the considered commit before the change.                                      \\
  & FIX & Whether or not the change is a defect fix. \\
  & NDEV & The number of developers that changed the modified files. \\
                                                                              &  AGE      &  The average time span between the last and the current change.                                                                 \\
                                                                              & NUC      & The number of times the file has been modified alone up to considered commit.                                                  \\
                                                                              &  CEXP     &  The number of commits performed on the given file by the committer up to the considered commit.                                \\
                                                                              & REXP     & The number of commits performed on the given file by the committer in the last month.                                          \\
                                                                              &  SEXP     &  The number of commits performed by a given developer in the considered package that contains the given file.                   \\
\hline 
\end{tabular}
% }
\caption{Product and process metrics proposed by Rahman~\cite{rahm2013} and Kamei~\cite{kamei2012large}}
\label{tab:jit-metrics}
\end{table*}
